User configurable 3D object regeneration for spatial privacy

Environmental understanding capability of $\textit{augmented}$ (AR) and $\textit{mixed reality}$ (MR) devices are continuously improving through advances in sensing, computer vision, and machine learning. Various AR/MR applications demonstrate such capabilities i.e. scanning a space using a handheld or head mounted device and capturing a digital representation of the space that are accurate copies of the real space. However, these capabilities impose privacy risks to users: personally identifiable information can leak from captured 3D maps of the sensitive spaces and/or captured sensitive objects within the mapped space. Thus, in this work, we demonstrate how we can leverage 3D object regeneration for preserving privacy of 3D point clouds. That is, we employ an intermediary layer of protection to transform the 3D point cloud before providing it to the third-party applications. Specifically, we use an existing adversarial autoencoder to generate copies of 3D objects where the likeness of the copies from the original can be varied. To test the viability and performance of this method as a privacy preserving mechanism, we use a 3D classifier to classify and identify these transformed point clouds i.e. perform $\textit{super}$-class and $\textit{intra}$-class classification. To measure the performance of the proposed privacy framework, we define privacy, $\Pi\in[0,1]$, and utility metrics, $Q\in[0,1]$, which are desired to be maximized. Experimental evaluation shows that the privacy framework can indeed variably effect the privacy of a 3D object by varying the privilege level $l\in[0,1]$ i.e. if a low $l<0.17$ is maintained, $\Pi_1,\Pi_2>0.4$ is ensured where $\Pi_1,\Pi_2$ are super- and intra-class privacy. Lastly, the privacy framework can ensure relatively high intra-class privacy and utility i.e. $\Pi_2>0.63$ and $Q>0.70$, if the privilege level is kept within the range of $0.17<l<0.25$.

==> 05-Evaluation-Setup.tex <==
\section{Experimental Setup}
\label{sec:Evaluation Setup}
\amaya{Shall we rename this section as Experiment setup?}

\subsection{Dataset}\label{sec:dataset}

% We have used a point cloud dataset where each point cloud was sampled from a mesh model of ShapeNetCore \amaya{(is it a derivation from original shapenet? should we cite that?)} with (area) uniform sampling\cite{achlioptas2017latent_pc}. Specifically, we have focused on household items i.e. bathtub, chair, monitor, sofa, table, bench, cabinet, bed, bookshelf and lamp. We have avoided large non-household objects like airplane, ship, etc. as it would be impractical for MR devices to capture these for a normal user.

For this work, we created a custom dataset by selecting a subset of the dataset introduced by \cite{achlioptas2017latent_pc} where 3D CAD models of ShapeNetCore \cite{shapenet2015} were sampled with (area) uniform sampling. Our dataset has 10 super-classes of household items i.e. \textit{bathtub, chair, monitor, sofa, table, bench, cabinet, bed, bookshelf and lamp}, with 100 unique object instances within each super-class. (We have avoided large non-household objects like airplane, ship, etc. as it would be impractical for MR devices to capture these for a normal user.) Every point cloud object was represented by 2048 points, and was normalized. 
\amaya{Training set privacy framework training was prepared by adding augmentations (random rotations and Gaussian noise) to the said data as explained in the following sections.  - take this part somewhere else}

\subsection{Adversarial attacker realization/simulation}\label{sec:Adversarial attacker realization/simulation}

In \S\ref{sec:Adversary models} , we discussed the theoretical framework and the hypothesis formulation used by an adversarial attacker to infer details about a point cloud at both \textit{super-class} and \textit{intra-class} level. In this section, we will discuss the practical simulation of such attackers in various scenarios and using them to evaluate our privacy framework effectiveness.

%Each adversary will form their hypothesis based on the data they have as a set of reference 3D objects. This reference data can be collected in various ways like using publicly available data, intercepting data from the same or different users or obtaining data via potentially colluding applications.

Both \textit{super-class} and \textit{inter-class} adversarial inference is done with respect to a set of reference 3D objects that are previously encountered and learnt from by the attacker in one or many of the following ways; From publicly available data, from the data intercepted previously from the same user or different users, or data obtained via other potentially colluding applications. In a situation where the query object is not present in the references (ie, not previously encountered by the attacker), the attacker attempts to identify the query as the structurally closest (most similar) reference object.

In our evaluation setup, we have used 10 super-classes \textit{(bathtub, chair, monitor, sofa, table, bench, cabinet, bed, bookshelf, lamp)} and 100 unique objects within each super-class as attacker's reference dataset. For our evaluation setup, we have $K = 10$ and $M_k = 100$ in \autoref{superclass_set}) and \autoref{subclass_set} respectively \amaya{Revise once Jaybie has finalized the notations}. 

%The labels for the complete dataset remain the same for each attacker but the way it is collected differ. 
We define the following four types of attackers based on the approach of acquiring and the quality of 3D data in their reference sets.
\begin{enumerate}
    \item $J_1$ - \textbf{public-aware attacker} -Using publicly available data as a set of reference 3D objects
    \item $J_1$ - \textbf{low-privilege-aware attacker} -Intercepting data from users with low privilege settings 
    \item $J_1$ - \textbf{medium-privilege-aware attacker} -intercepting data from users with medium privilege settings 
    \item $J_1$ - \textbf{high-privilege-aware attacker} -Intercepting data from users with high privilege settings 
\end{enumerate}

Given the difference in how attacker $J_1$ and attackers $J_2$,$J_3$ and $J_4$ learn their reference sets, two types of privacy threats can be identified. Attackers $J_2$,$J_3$ and $J_4$ are only exposed to regenerated point clouds from the proposed framework, therefore they lack knowledge about the unique objective features of the original point cloud object. The inference of a query point cloud $S^*$ by attackers $J_2$,$J_3$ and $J_4$ can be identified as an object reidentification attack; where the query can be identified with one of reference objects, but the attacker cannot derive further features or pose additional threats since the reference objects do not necessarily resemble their original counterparts. But on the other hand, attacker $J_1$ learns its reference set from publicly available data, where additional object, semantic, and contextual features are also possibly available for a given object. Once attacker $J_1$ infers a query point cloud $S^*$ with respect to such a reference set, in addition to an object reidentification threat, revealing the true identity of the object can lead to multiple other privacy threats. 


\subsubsection{Simulating attacker training process}
We created the reference dataset for the attacker $J_1$ by using publicly available dataset as mentioned in \S\ref{sec:dataset}. To effectively For each unique object in all the superclasses, we normalized the point cloud and added random Gaussian noise to create 100 point clouds.

\rsout{ To simulate the attackers, we created the reference dataset for each attacker by adding augmentations. This process can be considered as the attacker intercepting the data from real users or using publicly available data. }

\amaya{take this part to next subsubsection}
We used our privacy framework to create 100 reconstructions of each unique object from various privacy levels and used them as the reference dataset.

\amaya{brought from \S\ref{sec:3D Privacy Framework}

every other epoch i.e. all the even epoch numbers. We trained the framework for 300 epochs, so we have 150 saved weights in our weight bank.}

As explained in \S\ref{sec:point-cloud-transformations-for-different-privacy-levels}, the training epoch number from which the hypernetwork weights are loaded for point cloud transformation has an inverse proportional relationship with the provided privacy level. Therefore, we divided the available privacy levels to three abstract privacy settings based on the epoch ranges. 
(1) Low privacy - epoch range [70,300]
(2) Medium privacy - epoch range [50,70]
(3) High privacy - epoch range (0,50]
\jaybie{We mentioned in 4.2 that the privacy slider has values from 0 to 100, we might want to explain how that translates to these epoch values.}



For the attacker 2, we randomly chose 100 epochs within the range (0,50] with replacement and reconstructed each unique object. Similar procedure was followed for the attacker 3 and 4 except the range was changed to [50,70] and [70,300] respectively. The reference dataset generation for a single superclass ("Chair") is shown in the Fig. \ref{fig:attacker-training-dataset}.

\begin{figure}[h!]
	\centering
	\includegraphics[width=1\columnwidth]{figures/Attacker training dataset.pdf}
	\caption{Reference (training) dataset generation for the superclass "Chair"}
	\label{fig:attacker-training-dataset}
\end{figure}

Now, for each attacker, we have a reference dataset of size $10 \times 100 \times 100$ i.e. 100 reconstructions of each of the 100 unique objects for all the 10 super-classes. The attacker uses this reference data for training and validation of their classification models which helps them to infer the superclass and intraclass attributes of the query point cloud. In this work, we used the \textit{PointNet} neural network architecture as the 3D point cloud classifier \cite{qi2017pointnet}. For superclass classification, each attacker trains one classification model which uses the labeled dataset of size $10 \times 100 \times 100$ where we have $100 \times 100$ samples for each superclass. For intraclass classification, each attacker trains 10 classification models i.e. one for each superclass. Each of these 10 models uses the dataset of size $100 \times 100$, where we have 100 labeled samples (reconstructions) for each unique object. An attacker's classifier training process is shown in the Fig. \ref{fig:attacker-classifier-training}.

\begin{figure}[h!]
	\centering
	\includegraphics[width=1\columnwidth]{figures/Attacker models training.pdf}
	\caption{An attacker's classifier training process}
	\label{fig:attacker-classifier-training}
\end{figure}

\subsubsection{Evaluating the attacker performance}
To assess each attacker's success, we have to test all of their classification models against a real world scenario where a user uses our privacy framework. As discussed in \S\ref{sec:point-cloud-transformations-for-different-privacy-levels}, according to the user input on the privacy slider we choose an epoch from the range (0,300] and load the corresponding weights in our framework. This network is used to create a reconstruction of the original point cloud with the required privacy by the user. 

For each of the 100 unique objects from all the 10 superclasses, we created 3 reconstructions at every other epoch i.e. all the even numbered epochs in the range (0,300]. This labeled dataset of size $10 \times 100 \times 150 \times 3$​​​ was used to test all the 11 classifiers trained by each attacker. Our testing dataset will allow us to assess the attacker's success at inferring both the superclass and the intraclass attribute at various levels of privacy set by a normal user. Different random seeds were used while creating the testing and the training dataset using our privacy framework. The testing dataset generation for a single superclass ("Chair") is shown in the Fig. \ref{fig:attacker-testing-dataset}.

\subsection{Attacker hypothesis formulation}

The attackers that we realize in the form of 3D point cloud classifiers formulate two consecutive hypotheses for a query point cloud as explained in \autoref{hypothesis 1} and \autoref{hypothesis 2}. In this section we will elaborate the hypothesis formulation process taken by \textit{Pointnet} based classifiers. 

At the last activation function of Pointnet, the softmax layer outputs the probability distribution over predicted reference classes. We use this softmax output to define the scoring function in \autoref{Eq: Scoring function 1}.
%this output as a scoring function $E_{1}$ that generates a score for each reference class $c_{k}$ for a query

%\jaybie{By the way, I updated autoref for equations so you may just use autoref and `Eq.' will automatically be added.}

%\arpit{I think we should replace K=10 and Mk=100 in the following equations}
%\amaya{refer to equations from section 3}
$$E_{1}\left( S^{*} ,c_{k}\right) ,\ \forall c_{k} \in \upGamma ,\ |\upGamma |=K=10$$
% s.t,
% $$\sum _{k=1}^{K} E_{1}\left( S^{*} ,c_{k}\right) =1$$

Next, the attacker formulates the hypothesis in \autoref{hypothesis 1} by solving the following optimization. 
% $$\overline{\gamma } \in \gamma _{all}$$
\begin{equation}\label{Eq:hypothesis 1 optimization}
    \hat{C}\left( S^{*}\right) =\gamma =\ \underset{\overline{\gamma } \in \gamma _{all}}{\mathrm{Argmax}} \ \sum _{c_{k} \in \overline{\gamma }} E_{1}\left( S^{*} ,c_{k}\right)
\end{equation}

Similarly in the next step, we use the softmax output of the intra-class classifier trained on a particular super-class $c_{k}$ to formulate the scoring function in \autoref{Eq: Scoring function 2},

$$E_{2}\left( S^{*} ,d_{k,m} |c_{k}\right) ,\ \forall d_{k,m} \in \upDelta _{k} ,|\upDelta _{k} |=M_{k} =100\ $$
%s.t,
%$$\sum _{m=1}^{M} E_{2}\left( S^{*} ,d_{k,m} |c_{k}\right) =1$$

and formulates the hypothesis in \autoref{hypothesis 2} by solving the following optimization.
%$$\overline{\delta }_{k} \subset \delta _{k,all} \ $$
\begin{equation}\label{Eq:hypothesis 2 optimization}
    \hat{D}\left( S^{*}\right) |c_{k} =\delta _{k} =\ \underset{\overline{\delta }_{k} \subset \delta _{k,all} \ }{\mathrm{Argmax}} \ \sum _{d_{k,m} \in \overline{\delta }_{k}} E_{2}\left( S^{*} ,d_{k,m} |c_{k}\right)
\end{equation}

Note that the cardinalities of the subsets $\gamma$ and $\delta_{k}$ obtained in \autoref{Eq:hypothesis 1 optimization} and \autoref{Eq:hypothesis 2 optimization} are parameterized by $n_{1}$ and $n_{2}$ as shown in \autoref{hypothesis 1} and \autoref{hypothesis 2}. We evaluate the performance of our attackers with respect to these parameters in \S\ref{sec:Results}.

\begin{figure}[h!]
	\centering
	\includegraphics[width=1\columnwidth]{figures/Attacker testing dataset.pdf}
	\caption{Testset generation for the superclass "Chair"}
	\label{fig:attacker-testing-dataset}
\end{figure}

\subsection{Evaluation of point cloud Utility}\label{sec:Evaluation of point cloud Utility}

%\amaya{Shall we move this directly to the results section?} \jaybie{We can have a discussion here on how the utility is measured. In the results section, we show the results plus insights.}

Higher privacy usually comes at a cost of usability. The privacy framework should be able to deliver the MR application functionality while preserving the privacy of the point cloud objects. 
To this end, we utilize the three utility metrics defined in \S\ref{sec:utility metrics} 

In order to realize the utility metric $Q_{1:S,\Bar{S}}$ from \autoref{Utility metric 1}, we calculated the axis-aligned bounding boxes for each original point cloud $S$ and compared it with the bounding boxes from transformed point clouds $\Bar{S}$ for each privacy level. To remove the biases due to varying sizes of objects, we first normalized the point cloud $S$, and applied the transformations to it. \amaya{Are we including utility metric 1?}

Next, to realize the utility metric $Q_{1:S,\Bar{S}}$ from \autoref{Utility metric 1}, we used a modified implementation of RANSAC \cite{RANSACFischlerandMartin} algorithm to derive the most prominent 2D plane of each point cloud object. Since our dataset consists primarily of household objects, we conducted our analysis for 2D horizontal planes, e.g. sitting plane of chairs where virtual objects are most likely to be anchored on. But the utility metric $Q_{1:S,\Bar{S}}$ can be applied to any type of plane of choice. We obtain a set of points $p$ that are fitted to the most prominent 2D plane of the object by the RANSAC algorithm, and calculate the metrics given in the \autoref{Utility metric 2} separately for static and dynamic anchoring cases. To remove potential biases due to relative sizes of measurements of the four components of weighted addition in \autoref{Utility metric 2}, we normalized the individual distributions for each component;

$$|1-\overrightarrow{n_{p}} .\overrightarrow{n_{\overline{p}}} |,|\underline{r}_{p} -\underline{r}_{\overline{p}} |,|A( p) -A(\overline{p}) |,CD( p,\overline{p})$$

The third utility metric in \autoref{Utility metric 3} directly calculates the output transformation between $S$ and $\Bar{S}$ using Chamfer distance.
Chamfer pseudo-distance is a widely used metric to measure discrepancy between two point clouds. 
%Strictly speaking, it is not a distance function because the triangle inequality does not hold, hence the use of term "pseudo-distance". 
From the \autoref{hypercloud_cost}, it was also a part of the cost function in our framework. It measures the squared distance between each point in one point cloud to its nearest neighbor in the other point cloud:

\begin{equation}
    CD(X_1, X_2) = \sum_{x \in X_1} \underset{y \in X_2}{min} ||x-y||_2^2 + \sum_{x \in X_2} \underset{y \in X_1}{min} ||x-y||_2^2
\end{equation}

%\textcolor{red}{Some details about RANSAC}.\cite{RANSACFischlerandMartin}

\amaya{Brought from section 3 utility metrics

The third functionality $G_{3}$ requires a near-truth representation of the structure of the object.% as the functionality output. 
Hence, we define the Error $E_3$ as the \textit{Chamfer distance} between the original point cloud and the transformed point cloud.
Since Chamfer distance itself gives a clear definition for the discrepancy between $S$ and $\Bar{S}$, we will use $Er_{3:S,\overline{S}}$ itself in our analysis of regenerated point cloud utility.

$$G_{3} \rightarrow Y_{3,S} :S,\ Y_{3,\overline{S}} :\overline{S}$$
\begin{equation}\label{Utility metric 3}
    Er_{3:S,\overline{S}} =CD( S,\overline{S})
\end{equation}
}


==> 09-final_sections.tex <==
\section{MR Privacy Framework}%{Theoretical Framework}
\label{sec:framework}

\subsection{MR processing pipeline}



\subsection{\textbf{Why 3D?}}%\label{subsec:3d-data}With images and video, what the machine sees is practically what the user sees and a great deal of privacy work have been done on these data forms. Contrariwise, in MR, the experience is exported as visual data (e.g. objects augmented on the user's view) while its 3D nature, especially of the underlying data, is not exposed to the users: what the machine sees is different (arguably, even more) than what the user sees. That is, the digital representation of the physical world, the 3D point cloud data, is not exposed to the user. This inherent perceptual difference creates a disconnect and, perhaps, affects (or the lack thereof) how users perceive the sensitivity of 3D information. %Despite 3D data being a structural representation of the real world, 3D data is latent from user perception.
Furthermore, current MR platforms (i.e. Windows MR, ARCore and ARKit) directly operates on these 3D spatial maps or point clouds and, so far, no privacy preservation is applied before providing these data to third party applications.

\paragraph{\textbf{3D Point Cloud Data.}} The 3D points comprising the 3D point cloud can be described by their $\{x, y, z\}$-position in space with an accompanying normal vector $\{n_x, n_y, n_z\}$. Fig. \ref{fig:3D-privacy-problem} shows the point clouds as a mesh of 3D points with associated orientations represented by normal vectors. ...

\subsection{Adversary Model}\label{subsec:threat}

Adversaries may desire to, at the very least, infer the location of the users using released 3D data. They may further infer user poses, movement in space, or, even, detect changes in user environment. ...

\subsubsection{Deep-learning 3D inference} ...

\subsection{3D MR data}\label{subsec:3d-mr-data}

%\paragraph{Gathering sample data.}
We gathered real 3D point cloud data using the Microsoft HoloLens in an office environment to demonstrate the leakage from actual human-scale spaces in which an MR device is usually used.\footnote{There are numerous 3D point cloud datasets such as those listed in http://cvgl.stanford.edu/resources.html but most of these available 3D data sets are models of objects or of city-scale models.} %HoloLens hardware details at https://developer.microsoft.com/en-us/windows/mixed-reality/HoloLens\_hardware\_details}.

\subsubsection{3D transformations}

\section{Evaluation Setup}\label{sec:methodology}%Step 0: Privacy Leakage in 3D}\label{progress2}
%For our evaluation, we use the dataset described in \ref{subsec:3d-mr-data}. %We, first, introduce the spatial abstraction techniques in \S\ref{subsec:strategies}. Then, we describe the specific experimental setups in \S\ref{subsec:attack} which demonstrates adversarial inference to reveal 3D spaces which leads to spatial privacy leakage.

%\textcolor{red}{INCLUDE: (1) re-introduce the dataset, environment, etc. (2) the number of iterations, rotations, radii, (3) specific test cases , etc.}

%\subsection{Na\"ive Abstraction Strategies and Inference}\label{subsec:abstraction-strategy}

For evaluating the performance of an adversary as described in \S\ref{subsec:threat}, we check its inference performance over released modified point clouds. We use the descriptor set extracted from the 3D raw point cloud data as the reference set available to the adversary (labelled 1 in Fig. \ref{fig:adversary-model-pipeline}). We, then, implement various information reduction techniques to investigate how well can the adversary infer the identity, i.e. spatial location, of the released and modified point cloud.

\subsection{3D Segmentation} ...

\begin{figure}[t]
	\centering
	\vspace{-2mm}
	\includegraphics[width = \columnwidth]{figures/generalization_sample-8}
	\vspace{-3mm}
	\caption{\small Surface generalization, i.e. plane fitting, example: \small{(left) sample raw space, (center) RANSAC generalization, and (right) locally-originated generalization.}}
	\label{fig:generalization-example}
	\vspace{-5mm}
\end{figure}
%\textcolor{red}{Why generalize? True points and the generalized spaces.}
%
%Directly releasing raw point clouds exposes all spatial information.
To limit the amount of information released with the point clouds, (1) plane generalizations and (2) partial releasing can be utilised to provide MR applications the least information necessary to deliver the desired functionality. 
%We present two major protection strategies, (1) partial spaces, and (2) generalizations, and their combinations as well as successive release of spatial data using these strategies.

\subsection{3D Transformation} ...

\section{Results and Discussion}\label{sec:discussion}

In the succeeding discussions, we would like to emphasize the trends and relative values rather than absolute empirical values themselves. We also presented takeaways whose discussions on trends and relationships can be generalized. ...

\paragraph{\footnotesize\textbf{Takeaway.}} {\footnotesize \textit{...}}

\subsection{Computing utility post-transformation}
\label{subsec:utility-results}

Transformation contribute variations to the released point clouds from the original point clouds ... 

\subsection{Impact of transformation on utility}

IOU

\paragraph{\footnotesize\textbf{Takeaway.}} {\footnotesize \textit{Utility ...}}


\section{Limitations and Future Work}\label{sec:future_work}
In this work, we have only used \textit{geometric information}, i.e. point location $\{x,y,z\}$ and their normals $\{n_x,n_y,n_z\}$, but point cloud data may also include \textit{photometric information}, such as color, hue, light intensity, and so on. Further extensive analysis and investigation needs to be done over these extensions of the data. ...

\section{Conclusion}\label{sec:conclusion}

%Due to the rise in \textit{mixed reality} (MR) applications and devices in recent years, it is opportune to investigate the privacy and security issues that come with the technology.

In this work, we demonstrated how we can transform ... for privacy ...

In our future work, we aim to develop a ...

%\footnote{https://developers.google.com/ar/reference/java/arcore/reference/com/\\google/ar/core/PointCloud}

%\footnote{https://developer.apple.com/documentation/arkit/arpointcloud}



%\section*{Acknowledgments}  The authors would like to thank *** for providing insights through application activity and network packet analysis of MR applications running in HoloLens, Android's ARCore, and Apple's ARKit.
%  Dr. Yuhua Li for providing the
%  MATLAB code of the \textit{BEPS} method.
%
%  The authors would also like to thank the anonymous referees for
%  their valuable comments and helpful suggestions. The work is
%  supported by the \grantsponsor{GS501100001809}{National Natural
%    Science Foundation of
%    China}{http://dx.doi.org/10.13039/501100001809} under Grant
%  No.:~\grantnum{GS501100001809}{61273304}
%  and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
%    Scientists' Support Program}.

\begin{appendix}
\small
\section{3D transformation and preliminary evaluation}

\end{appendix}





==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       
